Memory of Motion for Warm-starting Trajectory Optimization

Trajectory optimization for motion planning requires good initial guesses to obtain good performance. In our proposed approach, we build a memory of motion based on a database of robot paths to provide good initial guesses. The memory of motion relies on function approximators and dimensionality reduction techniques to learn the mapping between the tasks and the robot paths. Three function approximators are compared: $k$-Nearest Neighbor, Gaussian Process Regression, and Bayesian Gaussian Mixture Regression. In addition, we show that the memory can be used as a metric to choose between several possible goals, and using an ensemble method to combine different function approximators results in a significantly improved warm-starting performance. We demonstrate the proposed approach with motion planning examples on the dual-arm robot PR2 and the humanoid robot Atlas.

==> sections/problem_formulation.tex <==
\section{Problem formulation}
\label{sec:problem_formulation}

The aim of robot motion planning is to obtain a sequence of robot configurations that accomplishes a certain task, e.g. to move from a starting to a goal configuration while avoiding obstacles. If the configuration sequence is parameterized by time, it is called trajectory, otherwise it is called path. Trajectory optimization gains popularity in the motion planning community due to its ability to handle arbitrary constraints and high dimensionality. Denoting the robot configuration at timestep $t$ as $\bm{q}_t \in \mathbb{R}^{D}$, where $D$ is the robot's DoFs, trajectory optimization formulates the motion planning problem as an optimization problem,
%
\begin{equation}
\min_{\bm{q}_{0:T}} \ell ( \bm{q}_{0:T}), \quad ~\text{s.t.}~ \bm{g}( \bm{q}_{0:T}) \leq \bm{0},\quad \bm{h}( \bm{q}_{0:T}) = \bm{0},
\label{eq:minimization}
\end{equation}
%
%\begin{equation}
%~\text{s.t.}~ g_i( \bm{q}_{0:T}) \leq \bm{0},\quad h_j( \bm{q}_{0:T}) = \bm{0},
%\end{equation}
%
where $\bm{q}_{0:T}$ denotes the robot's configurations at the timestep $t = 0$ to $t = T$, $\ell (\cdot), \bm{g}(\cdot)$, and $\bm{h}(\cdot)$ are the cost, the inequality constraints, and the equality constraints. The solution of~\eqref{eq:minimization} is the path $\bm{y} = {\bm{q}_{0:T}}^{\ast} = ( \bm{q}_{0}^{\ast \top}, \dots, \bm{q}_{T}^{\ast \top})^\top \in \mathbb{•}{R}^{DT}$. 

For example, if the task $\bm{x}$ is to move from an initial to a goal configuration (i.e. $\bm{x} = (\bm{q}_\text{init}^\top,\bm{q}_\text{goal}^\top)^\top$) while minimizing the total joint velocity, the optimization problem can be written as
%cost
\begin{equation}
\min_{\bm{q}_{0:T}} \sum{}_{t=0}^{T-1}  \left\Vert(\bm{q}_{t+1} - \bm{q}_{t})\right\Vert ^2 \quad ~\text{s.t.}~ \bm{q}_{0} = \bm{q}_{init}, \quad \bm{q}_{T} = \bm{q}_{goal}
\label{eq:discrete_vel}
\end{equation}
%\begin{equation}
%~\text{s.t.}~ \bm{q}_{0} = \bm{q}_{init}, \quad \bm{q}_{T} = \bm{q}_{goal}
%\end{equation}
%
Other constraints can also be added, e.g. to avoid collision, to comply with joint limit, etc. 

Such optimization problems are in general non-convex, especially due to the collision constraints, which makes finding the global optimum very difficult. Trajectory optimization methods such as TrajOpt \cite{schulman2013finding}, AICO \cite{toussaint2009robot}, CHOMP \cite{zucker2013chomp}, STOMP \cite{kalakrishnan2011stomp}, or ITOMP \cite{park2012itomp} typically solve the non-convex problem by iteratively optimizing around the current solution. 
%iterative methods such as Sequential Quadratic Programming(SQP). At each iteration, the method constructs a convex approximation to the original optimization problem around the current solution which can be solved easily. 
While such approach is very popular and yields good practical results, the convergence and the quality of the solution are very sensitive to the choice of initial guess. If the initial guess is far from the optimal solution, the method can get stuck at a poor local optimum.

To overcome this problem, our approach is to build a \emph{memory of motion} that learns how to provide a good initialization (i.e. \emph{warm-start}) to the solver based on previously solved problems. Building the memory of motion can be seen as learning a mapping from a given task to the associated robot path. Our proposed method rely on machine learning techniques such as function approximation and dimensionality reduction to learn this mapping effectively, as explained in the next section. 

%This idea presents the following benefit:
%\begin{itemize}
%\item It follows the principle of 'do not reinvent the wheel'. If a similar problem has been previously solved, this should be used as an initial guess for different but similar problems.
%\item Since the memory of motion can be built offline, we can spend a lot of time and effort to build a high-quality memory of motion, e.g. with various initialisation methods and carefully-engineered heuristics. 
%\item The memory of motion can be used not only as an initial guess, but also to provide a metric in the case of multiple goals. The memory can provide an initial guess for each potential goal, and we can evaluate these initial guesses to select the goal that may give us the best result without actually solving each problem. 
%\end{itemize}

%
%\begin{figure}
%\centering
%\includegraphics[width=0.4\columnwidth]{bd_regression.pdf}
%\caption{The memory of motion approximates the mapping between the task descriptor $\bm{x}$ and the robot path $\bm{y}$ using the database of motions}
%\label{fig:bd_regression}
%\end{figure}





==> sections/suplementary.tex <==
\section{Supplementary Materials}
\label{sec:supplement}

\subsection{Bayesian Gaussian Mixture Regression (BGMR)}
As discussed in the main text, given the training dataset $\{\bm{X},\bm{Y}\}$ GMR constructs the joint probability of $(\bm{x},\bm{y})$ as a mixture of Gaussians,
%
\begin{equation}
p(\bm{x},\bm{y}) = \sum_{k=1}^K \pi_k \, \mathcal{N}(\bm{\mu}_k,\bm{\Sigma}_k),
\end{equation}	
%
where $\pi_k$, $\bm{\mu}_k$, and $\bm{\Sigma}_k$ are the $k$-th component's mixing coefficient, mean, and covariance, respectively. Let $\bm{\theta} = \{\pi_k,\bm{\mu}_k, \bm{\Sigma}_k\}_{k=1}^K$, denoting the GMR parameters to be determined from the data. 

We can decompose $\bm{\mu}_k$ and $\bm{\Sigma}_k$ according to $\bm{x}$ and $\bm{y}$ as
\begin{equation}
\bm{\mu}_k = \begin{pmatrix} \bm{\mu}_{k,x} \\ \bm{\mu}_{k,y} \end{pmatrix} \quad \text{and} \quad \bm{\Sigma}_k = 
\begin{pmatrix}
\bm{\Sigma}_{k,xx} & \bm{\Sigma}_{k,xy} \\
\bm{\Sigma}_{k,yx} & \bm{\Sigma}_{k,yy}
\end{pmatrix}.
\end{equation}
%
Given a query $\bm{x}^*$, the predictive distribution of $\bm{y}$ can then computed by conditioning on $\bm{x}^*$, 
%
\begin{equation}
p(\bm{y}|~\bm{x}^*,\bm{\theta}) = \sum_{k=1}^K p(k|~\bm{x}^*,\bm{\theta}) \, p(\bm{y}|~k,\bm{x}^*,\bm{\theta}), 
\label{eq:gmr_pred_sup}
\end{equation}
%
where $p(k|~\bm{x}^*,\bm{\theta})$ is the probability of $\bm{x}^*$ belonging to the $k$-th component, 
\begin{equation}
p(k|~\bm{x}^*,\bm{\theta}) = \frac{\pi_k \, \mathcal{N}(\bm{x}^* |~ \bm{\mu}_{k,x}, \bm{\Sigma}_{k,xx})}{\sum_{i=1}^{K} \pi_i \, \mathcal{N}(\bm{x}^* |~ \bm{\mu}_{i,x}, \bm{\Sigma}_{i,xx}) },
\label{eq:prob_k}
\end{equation}
and $p(\bm{y}|~k,\bm{x}^*,\bm{\theta}$) is the predictive distribution of $\bm{y}$ according to the $k$-th component, 
\begin{equation}
p(\bm{y}|~k,\bm{x}^*,\bm{\theta}) = \mathcal{N}\Big(\bm{\mu}_{k,y} + \bm{\Sigma}_{k,yx} {\bm{\Sigma}^{-1}_{k,xx}}(\bm{x}^* - \bm{\mu}_{k,x}), \; \bm{\Sigma}_{k,yy} - \bm{\Sigma}_{k,yx} {\bm{\Sigma}^{-1}_{k,xx}} \bm{\Sigma}_{k,xy}\Big),
\label{eq:pred_k}
\end{equation}
%
which is a Gaussian distribution with the mean being linear in $\bm{x}^*$. The resulting predictive distribution \eqref{eq:gmr_pred_sup} is then a mixture of Gaussians. 

In GMR, $\bm{\theta}$ is usually estimated from the dataset $\{\bm{X},\bm{Y}\}$ by using Expectation-Minimization method that outputs a single value for $\bm{\theta}$, and the prediction is computed using this value. Instead, Bayesian GMR (BGMR) puts priors to the parameter $\bm{\theta}$, and given the dataset $\{\bm{X},\bm{Y}\}$, it computes the posterior distribution $p(\bm{\theta} |~\bm{X},\bm{Y})$. Hence, when we do prediction we have to integrate over the posterior distribution of $\bm{\theta}$, 
\begin{equation}
p(\bm{y}~|~\bm{x}^*, \bm{X},\bm{Y} ) = \int_{\bm{\theta}}^{} p(\bm{y}~|~\bm{x}^*, \bm{\theta}) \, p(\bm{\theta} ~|~ \bm{X},\bm{Y}) \, d\bm{\theta}. 
\label{eq:integrate_post}
\end{equation}
%
The resulting predictive distribution is then a mixture of multivariate t-distributions, 
\begin{equation}
p(\bm{y}~|~\bm{x}^*, \bm{X},\bm{Y}) = \sum_{k=1}^K p(k~|~\bm{x}^*, \bm{X},\bm{Y}) \, p(\bm{y}~|~k,\bm{x}^*,\bm{X},\bm{Y}), 
\label{eq:bgmr_pred_sup}
\end{equation}
where $p(k\,|\,\bm{x}^*, \bm{X},\bm{Y})$ is the probability of $\bm{x}^*$ belonging to the $k$-th component and $p(\bm{y}~|~k,\bm{x}^*,\bm{X},\bm{Y})$ is the predictive distribution of $\bm{y}$ according to the $k$-th component. These are calculated using the formula similar to \eqref{eq:prob_k} and \eqref{eq:pred_k}, but the Gaussian distributions are replaced by t-distributions. $p(\bm{y}~|~k,\bm{x}^*,\bm{X},\bm{Y})$ is a t-distribution (whose mean is also linear w.r.t.~$\bm{x}^*$) instead of a Gaussian distribution as in \eqref{eq:pred_k}, due to the integration over the posterior distribution in \eqref{eq:integrate_post}. 

%, 
%\begin{equation}
%p(k~|\bm{x}^*,\bm{\theta}) = \frac{\pi_k \mathcal{N}(\bm{x}^* ~| \bm{\mu}_{k,x}, \bm{\Sigma}_{k,xx})}{\sum_{i}^{K} \pi_i \mathcal{N}(\bm{x}^* ~| \bm{\mu}_{i,x}, \bm{\Sigma}_{i,xx}) }
%\end{equation}

%\begin{equation}
%p(\bm{y}^*~|k,\bm{x}^*,\bm{\theta}) = \mathcal{N}(\bm{\mu}_{k,y} + \bm{\Sigma}_{k,yx} {\bm{\Sigma}_{k,xx}}^{-1}(\bm{x}^* - \bm{\mu}_{k,x}), \bm{\Sigma}_{k,yy} - \bm{\Sigma}_{k,yx} {\bm{\Sigma}_{k,xx}}^{-1} \bm{\Sigma}_{k,xy}),
%\end{equation}

Note that the predictive distribution of GMR \eqref{eq:gmr_pred_sup} and BGMR \eqref{eq:bgmr_pred_sup} are very similar, but \eqref{eq:gmr_pred_sup} is a mixture of Gaussians whereas \eqref{eq:bgmr_pred_sup} is a mixture of t-distributions. Both can be seen as a mixture of linear regressions, since the mean prediction according to each $k$-th component \eqref{eq:pred_k} is linear in $\bm{x^*}$. 

The advantage of having a Bayesian version of GMR is the following:
\begin{itemize}
\item When the dimension of $\bm{x}$ and $\bm{y}$ is high, the number of parameters to be estimated in $\bm{\theta}$ is large and the estimation of $\bm{\theta}$ in GMR is prone to overfitting, unless the number of training data is very large. Putting the priors to $\bm{\theta}$ in BGMR helps mitigating the overfitting and makes it possible to learn with fewer number of datapoints.
\item By putting Dirichlet Process prior to the parameters $\pi_k$, the number of components $K$ can be determined automatically. 
\end{itemize}

To illustrate how BGMR can handle multimodal output, we show an illustrative example in Figure \ref{fig:toy_example}, which depicts a mapping $y = f(x)$ that is discontinuous at $x$ = 4 and $x$ = 6, and has two modes at $0 < x < 4$. The data points corresponding to $(x,y)$ are shown in black. First, BGMR fits a mixture of Gaussians to ($x,y$), shown as red ellipses in Figure \ref{fig:toy_example}a. We can see that the Gaussians fit well each mode and each side of discontinuity. 

Given a query point $x^*$, the predictive distribution of $y^*$ is a mixture of t-distributions given by \eqref{eq:bgmr_pred_sup}. Figure \ref{fig:toy_example}b shows an example of $p(y~|x)$ for $x = 0.8$. We can see that there are two peaks corresponding to the two modes of the mapping $f$ (i.e., $y$ = 25.2 and $y$ = 46.7), having roughly the same probability ($0.5$). 

Figure \ref{fig:toy_example}c shows the BGMR predictions over the range of $x$, by taking the mean of the components with the highest and the second-highest probability in \eqref{eq:bgmr_pred_sup}. We see that it predicts both modes very well, and it still performs well at discontinuous region (i.e., it does not average the both sides of discontinuity). 


\begin{figure}[t!]
\centering
\subfloat[][]{\includegraphics[width=0.3\columnwidth]{multi_modal_function}\label{fig:toy_example_a}}
\subfloat[][]{\includegraphics[width=0.3\columnwidth]{prob_y}\label{fig:toy_example_b}}
\subfloat[][]{\includegraphics[width=0.3\columnwidth]{bgmr_prediction}\label{fig:toy_example_3}}
\caption{
An example of multimodal and discontinuous mapping $f: x \rightarrow y$. BGMR fits a mixture of Gaussians to the joint data of $\bm{x}$ and $\bm{y}$ (a), resulting in a mixture of t-distributions as the predictive distribution of $y$ given $x^* = 0.8$ (b). By taking the means of the highest and second highest component of the mixture, BGMR approximates the mapping very well (c).}
\label{fig:toy_example}
\end{figure}		


%This is especially important for BGMR, since it needs to estimate the covariance matrix $\bm{\Sigma}_k$ which grows quadratically as the number of dimensions. 

%	- Discuss the storage and computational complexity (training and prediction)










% Experiment

%About TrajOpt
%TrajOpt applies sequential convex optimization to solve the motion planning problem. The collision avoidance in TrajOpt is implemented as soft constraint with an outer loop that increases the penalty weight if the constraints are not satisfied by the current solution. TrajOpt has two collision costs: discrete and continous. The discrete collision cost is based on the signed distance between the robot's links and the obstacles at the time step $t$, while the continuous collision cost consider the volume swept by the links between the time steps. The continuous collision cost enables TrajOpt to plan with much fewer time steps as compared to the other methods. However, it does not check self-collisions. We therefore use both costs in all our experiments.  
%
%In Section 4.1, the initial pose 
%
%
%In Section 4.2, the initial joint configuration is depicted in Figure ***, while the goal configuration is randomly sampled while 
%\td{The initial and goal configurations have both arms outside and inside the shelf, respectively}. 
%\td{In both configurations the hands are inside the shelf.} 
%
%while the orientations and the initial joint configurations are kept fix.

% Algorithm





